Testing new physics models with global comparisons to collider measurements: the Contur toolkit

Measurements at particle collider experiments, even if primarily aimed at understanding Standard Model processes, can have a high degree of model independence, and implicitly contain information about potential contributions from physics beyond the Standard Model. The Contur package allows users to benefit from the hundreds of measurements preserved in the Rivet library to test new models against the bank of LHC measurements to date. This method has proven to be very effective in several recent publications from the Contur team, but ultimately, for this approach to be successful, the authors believe that the Contur tool needs to be accessible to the wider high energy physics community. As such, this manual accompanies the first user-facing version: Contur v2. It describes the design choices that have been made, as well as detailing pitfalls and common issues to avoid. The authors hope that with the help of this documentation, external groups will be able to run their own Contur studies, for example when proposing a new model, or pitching a new search.

==> mkgenplots <==
#! /usr/bin/env bash

ROOT=$PWD
test "$GENS" || GENS=123
test "$STYLE" || STYLE=final

function mkplots() {
    FILE=$(basename $MAP)
    DIR=$(dirname $MAP)
    cd $DIR
    echo "In $PWD..."
    if [[ -e $FILE ]]; then
        echo $PWD && contur-plot $FILE mtp $KNAME -x '$M_Q$ (GeV)' -y '$\kappa$' --style=$STYLE -o . $@
    else
        echo "No contur.map file found" 1>&2
    fi
    echo
}

(echo $GENS | grep -q 1) && {
    echo "Generation 1"
    MAP=$ROOT/1Gen/HWZ001/contur.map GEN=1 KNAME=kappa mkplots -d $ROOT/flavlimits.py &
    MAP=$ROOT/1Gen/HWZ010/contur.map GEN=1 KNAME=kappa mkplots -d $ROOT/flavlimits.py &
    MAP=$ROOT/1Gen/HWZ100/contur.map GEN=1 KNAME=kappa mkplots -d $ROOT/flavlimits.py &
    MAP=$ROOT/1Gen/HWZ111/contur.map GEN=1 KNAME=kappa mkplots -d $ROOT/flavlimits.py &
    echo
    wait
}

(echo $GENS | grep -q 2) && {
    echo "Generation 2"
    MAP=$ROOT/2Gen/HWZ001/contur.map GEN=2 KNAME=kappa mkplots -d $ROOT/flavlimits.py &
    MAP=$ROOT/2Gen/HWZ010/contur.map GEN=2 KNAME=kappa mkplots -d $ROOT/flavlimits.py &
    MAP=$ROOT/2Gen/HWZ100/contur.map GEN=2 KNAME=KT mkplots -d $ROOT/flavlimits.py &
    MAP=$ROOT/2Gen/HWZ111/contur.map GEN=2 KNAME=KT mkplots -d $ROOT/flavlimits.py &
    echo
    wait
}

(echo $GENS | grep -q 3) && {
    echo "Generation 3"
    MAP=$ROOT/3Gen/HWZ001/contur.map GEN=3 KNAME=KT mkplots &
    MAP=$ROOT/3Gen/HWZ010/contur.map GEN=3 KNAME=KT mkplots &
    MAP=$ROOT/3Gen/HWZ100/contur.map GEN=3 KNAME=KT mkplots &
    MAP=$ROOT/3Gen/HWZ111/contur.map GEN=3 KNAME=KT mkplots &
    echo
    wait

    echo "Generation 3 no-correlations"
    MAP=$ROOT/3Gen/HWZ001/nocorr/conturNoCorr.map GEN=3 KNAME=KT mkplots &
    MAP=$ROOT/3Gen/HWZ010/nocorr/conturNoCorr.map GEN=3 KNAME=KT mkplots &
    MAP=$ROOT/3Gen/HWZ100/nocorr/conturNoCorr.map GEN=3 KNAME=KT mkplots &
    MAP=$ROOT/3Gen/HWZ111/nocorr/conturNoCorr.map GEN=3 KNAME=KT mkplots &
    wait
}

